Training-free Conditional Object Composition for Multi-object Image Generation with Diffusion Models

Multi-object image generation in text-to-image diffusion models remains challenging, as existing approaches struggle to reliably generate all objects specified in a prompt. Compositional approaches that generate objects independently often fail to capture the interactions among them, whereas joint generation methods tend to suffer from inter-object interference. In this work, we propose a training-free framework, termed conditional object composition, that relaxes joint generation methods by taking one step back toward compositional approaches. Our framework decomposes the generation of $N$ objects into two stages: it first generates a subset of $N-1$ objects and then composes the remaining object conditioned on the generated content. To enable effective composition, we adopt an inpainting-based formulation with layout guidance to preserve existing regions and encourage spatially coherent placement. To address the challenge of selecting which objects to generate separately, we introduce an attention-based scoring mechanism based on cross-attention maps and further explore the use of off-the-shelf object detectors. We evaluate our method on multi-object image generation using the widely adopted MS COCO dataset. Experimental results show that our approach achieves competitive or improved performance compared to existing methods, particularly as the number of objects increases. Further studies highlight the importance of the proposed design choices. The source code is available at https://github.com/ShampooWang/condComp_imageGen/tree/main

==> sections/preliminaries.tex <==
\section{Preliminaries}
\subsection{Text-to-image latent diffusion models}
Text-to-image latent diffusion models, such as Stable Diffusion~\cite{rombach2022sd} and SDXL~\cite{podellsdxl}, generate images by iteratively denoising a latent variable conditioned on a text prompt. Starting from Gaussian noise $\mathbf{z}_T \sim \mathcal{N}(0, \mathbf{I})$, the model performs a sequence of denoising steps to obtain a clean latent $\mathbf{z}_0$, which is then decoded into an image $\mathbf{x}_0$.

At each timestep $t$, the denoising process is guided by a neural network $\epsilon_\theta$ that predicts the noise component conditioned on the current latent $\mathbf{z}_t$ and a text embedding $\mathbf{c}$ extracted from the input prompt using a CLIP text encoder~\cite{radford2021clip}. The update can be written as

\begin{equation}
    \mathbf{z}_{t-1} = \mathcal{F}(\mathbf{z}_t, \epsilon_\theta(\mathbf{z}_t, t, \mathbf{c}))
    \label{eq:diffusion_update}
\end{equation}

where $\mathcal{F}$ denotes the sampling function determined by the chosen scheduler. To incorporate textual information, modern diffusion models employ cross-attention layers that fuse latent features with text embeddings. 

\subsection{Cross-Attention in Diffusion Models}
Cross-attention layers enable the interaction between spatial latent features and text tokens during the denoising process. At a given layer $l$, let $\mathbf{z}^{l} \in \mathbb{R}^{C \times H \times W}$ denote the latent feature map, and let $\{\mathbf{c}_m\}_{m=1}^{M}$ denote the token embeddings from the input prompt.

For each spatial location $u \in \{1, 2, \dots, H\} \times \{1, 2, \dots, W\}$ and token $j \in \{1, 2, \dots, M\}$, cross-attention computes an attention weight
\begin{equation}
    A^{l}_{uj} = 
    \frac{\exp\left(\langle Q^{l}_u, K^{l}_j \rangle\right)}
    {\sum_{m=1}^{M} \exp\left(\langle Q^{l}_u, K^{l}_m\rangle\right)},
\end{equation}
where $Q^{l}_u$ is the query of latent feature $z^l$ at spatial location $u$ and $K^{l}_j$ is the key corresponding to token $\mathbf{c}_j$.

The resulting cross-attention map $A^{l} \in \mathbb{R}^{H \times W \times M}$ provides a spatial map for each token. In particular, the map associated with token $j$ is denoted by $A^{l}_{:,:,j} \in \mathbb{R}^{H \times W}$. In practice, attention maps are often aggregated across multiple layers. For simplicity, we denote the aggregated attention map by $A$ and omit the layer index $l$ when no ambiguity arises.

These attention maps establish a correspondence between text tokens and spatial regions in the generated image. In this work, we focus on object-related tokens and utilize their attention maps to guide object composition and decomposition during inference.
